Design and Operation of Shared Machine Learning Clusters on Campus

Amid the rapid advancements in large machine learning (ML) models, universities worldwide are investing substantial funds and efforts into GPU clusters. However, managing a shared GPU cluster poses a pyramid of challenges, from hardware configuration to resource allocation among users. This paper introduces SING, a full-stack solution designed to streamline the management of shared GPU clusters in academic institutions. Motivated by the pressing need for efficient resource sharing and the challenges posed by limited staffing, we present a comprehensive view of SING's architecture and design choices, which achieves operational efficiency (i.e., low maintenance cost and high resource utilization). We also share experience and insights from the real-world operations of SING, including analysis of its usage patterns and management of incidents and failures. This paper is part of our ongoing effort to improve the management of shared ML clusters. We open-source relevant resources to facilitate the development and operation of similar clusters for ML.

==> sections/5-extension.tex <==
\section{Extensibility in \sys}
\label{section:extension}

This section explores potential extensions within the layers of \sys, including those with a research focus, as illustrated in Figure~\ref{figure:extension}.
These extensions provide a pathway to upgrade \sys's capabilities or performance when needed in cluster operation. 
Moreover, extensions in these layers can be seamlessly integrated beneath the job profile layer, and remain transparent to users.

\subsection{Extending the Adapter Layer}

The adapter layer handles two responsibilities~(\S\ref{section:design:layer2}): it offers a unified interface for users to submit jobs locally and injects environment provisioning scripts before submitting to schedulers. Opportunities are identified in these two steps.

\t{Cluster Selection.} 
On the client side of the adapter layer, running on the user's computer, there is a possibility for connecting job submissions to different clusters, each with a different computation infrastructure (discussed below). This provides users with a unified experience at a higher level: users can compose and test their jobs locally and then submit them to different clusters, which might be different in location, speed, or cost, without changing a single line of code. This concept is akin to serverless computing, where users are unaware of the actual computation's location and execution process.

\t{API-compatible Dependency Swap.} 
The transformations applied to job profiles also have the potential to impact the execution of jobs. 
During the environment provisioning stage, dependencies specified in the user's job profile can be replaced with API-compatible alternatives. 
A trivial example is, if the job's environment includes a PyTorch version compatible with the cluster's GPUs, users who initially tested their job locally with PyTorch on a CPU can seamlessly switch to a GPU-accelerated PyTorch version.
These API-compatible dependency replacements can yield more performance gains with recent research outcomes, such as collective communication APIs with platform-specific optimizations and utilizing hardware accelerators for specialized computations.

\subsection{Extending the Scheduler Layer}

Many cluster workload scheduling algorithms with different objectives exist~\cite{pollux, sia, gavel, optimus, themis}. 
We make a note that these schedulers primarily function as policies and lack workload manager capabilities, such as resource registration and release. As a result, these algorithms are typically implemented within cluster managers that provide the necessary mechanisms to realize the policies.

Among the scheduling algorithms, we introduce a particularly interesting direction, load shifting~\cite{loadshifting}. Load shifting involves rescheduling jobs with temporal flexibility to time periods when electricity costs are lower, or carbon density is reduced, reducing cluster-wide environmental impact, as illustrated in Figure~\ref{figure:extension}.
Research jobs, especially in training large models, often require hours or days to complete, thus exhibiting limited time sensitivity to minor progress variations. Therefore, schedulers can leverage this temporal elasticity to consume energy during off-peak times, achieving cluster-wide environmental objectives~\cite{carbon}.

\begin{figure}[t]
    \includegraphics[width=0.48\textwidth]{figures/figure-extension.pdf}
    \caption{\b{Examples of potential extensions for \sys clusters, highlighting opportunities in each layer.}}
    \vspace{-15pt}
    \label{figure:extension} 
\end{figure}

\subsection{Extending the Executor Layer}


The executor layer can be extended to, or federated~\cite{federation} with different computation backends, offering better scalability.

\t{Containerization on Kubernetes}. 
One potential extension is the integration of Docker containers within the Kubernetes~\cite{k8s} platform. This adaptation allows \sys to leverage Kubernetes' dynamic orchestration capabilities for managing containers. Users can seamlessly execute their jobs within Docker containers, benefiting from Kubernetes' scalability resource allocation features. 

\t{On-demand Cloud Computing Resource}.
Another intriguing possibility involves the integration of cloud-based compute nodes into the executor layer. With this extension, \sys could request cloud resources on-demand as part of the job submission process. This approach offers scalability and flexibility, allowing university computation facilities to offer additional computational power when needed.

These extensions, when co-designed with the adapter layers, can function transparently for users without requiring any code modifications. 
As a result, the computation backend can seamlessly extend to various types of resources, providing a serverless-like experience where users are unaware of the underlying infrastructure.









